AdaSmooth: An Adaptive Learning Rate Method based on Effective Ratio

It is well known that we need to choose the hyper-parameters in Momentum, AdaGrad, AdaDelta, and other alternative stochastic optimizers. While in many cases, the hyper-parameters are tuned tediously based on experience becoming more of an art than science. We present a novel per-dimension learning rate method for gradient descent called AdaSmooth. The method is insensitive to hyper-parameters thus it requires no manual tuning of the hyper-parameters like Momentum, AdaGrad, and AdaDelta methods. We show promising results compared to other methods on different convolutional neural networks, multi-layer perceptron, and alternative machine learning tasks. Empirical results demonstrate that AdaSmooth works well in practice and compares favorably to other stochastic optimization methods in neural networks.

==> symbols.tex <==
% Definitions of handy macros can go here
\newcommand{\dataset}{{\cal D}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}

\newcommand{\real}{\mathbb{R}}
\newcommand{\integer}{\mathbb{Z}}
%\newcommand{\det}{\mathrm{det}}

\newcommand{\cspace}{\mathcal{C}}
\newcommand{\nspace}{\mathcal{N}}

\newcommand{\leadto}{\qquad\underrightarrow{ \text{leads to} }\qquad}
\newcommand{\leadtosmall}{\,\,\underrightarrow{ \text{leads to} }\,\,}


%%%% NEW DEFINITIONS %%%%%

\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Exp}{\mathrm{E}}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\gap}{\,\,\,\,\,\,\,\,}


\newcommand{\exampbar}{\hfill $\square$\par}

%\newcommand{\bC}{\mat{C}}
%\newcommand{\ba}{\vec{a}}
%\newcommand{\bC}{\mathbf{C}}

%% begin new command fo clustering
\newcommand{\bOmega}{\boldsymbol\Omega}
\newcommand{\bomega}{\boldsymbol\omega}
\newcommand{\balpha}{\boldsymbol\alpha}
\newcommand{\bbeta}{\boldsymbol\beta}
\newcommand{\bdelta}{\boldsymbol\delta}
\newcommand{\btheta}{\boldsymbol\theta}
\newcommand{\bTheta}{\boldsymbol\Theta}
\newcommand{\bPhi}{\boldsymbol\Phi}
\newcommand{\bPsi}{\boldsymbol\Psi}
\newcommand{\bpsi}{\boldsymbol\psi}
\newcommand{\bgamma}{\boldsymbol\gamma}
\newcommand{\bepsilon}{\boldsymbol\epsilon}
\newcommand{\bLambda}{\boldsymbol\Lambda}
\newcommand{\boldeta}{\boldsymbol\eta}
\newcommand{\blambda}{\boldsymbol\lambda}
\newcommand{\bphi}{\boldsymbol\phi}
\newcommand{\bphiast}{\bphi_\ast}
\newcommand{\bmu}{\boldsymbol\mu}
\newcommand{\bsigma}{\boldsymbol\sigma}
\newcommand{\bSigma}{\boldsymbol\Sigma}


\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand{\diag}{\mathrm{diag}}


\newcommand{\dotL}{\dot{\bm{L}}}
\newcommand{\dotU}{\dot{\bm{U}}}
\newcommand{\ddotL}{\ddot{\bm{L}}}


%\newcommand{\widetildebG}{\widetilde{\bm{G}}}
%\newcommand{\widetildebV}{\widetilde{\bm{V}}}
%\newcommand{\widetildebU}{\widetilde{\bm{U}}}
%\newcommand{\widetildebv}{\widetilde{\bm{v}}}
\newcommand{\widebarbA}{\overline{\bm{A}}}
\newcommand{\widebarbB}{\overline{\bm{B}}}
\newcommand{\widebarbC}{\overline{\bm{C}}}
\newcommand{\widebarbD}{\overline{\bm{D}}}
\newcommand{\widebarbE}{\overline{\bm{E}}}
\newcommand{\widebarbF}{\overline{\bm{F}}}
\newcommand{\widebarbG}{\overline{\bm{G}}}
\newcommand{\widebarbH}{\overline{\bm{H}}}
\newcommand{\widebarbI}{\overline{\bm{I}}}
\newcommand{\widebarbJ}{\overline{\bm{J}}}
\newcommand{\widebarbK}{\overline{\bm{K}}}
\newcommand{\widebarbL}{\overline{\bm{L}}}
\newcommand{\widebarbM}{\overline{\bm{M}}}
\newcommand{\widebarbN}{\overline{\bm{N}}}
\newcommand{\widebarbO}{\overline{\bm{O}}}
\newcommand{\widebarbP}{\overline{\bm{P}}}
\newcommand{\widebarbQ}{\overline{\bm{Q}}}
\newcommand{\widebarbR}{\overline{\bm{R}}}
\newcommand{\widebarbS}{\overline{\bm{S}}}
\newcommand{\widebarbT}{\overline{\bm{T}}}
\newcommand{\widebarbU}{\overline{\bm{U}}}
\newcommand{\widebarbV}{\overline{\bm{V}}}
\newcommand{\widebarbW}{\overline{\bm{W}}}
\newcommand{\widebarbX}{\overline{\bm{X}}}
\newcommand{\widebarbY}{\overline{\bm{Y}}}
\newcommand{\widebarbZ}{\overline{\bm{Z}}}
\newcommand{\widebarba}{\overline{\bm{a}}}
\newcommand{\widebarbb}{\overline{\bm{b}}}
\newcommand{\widebarbc}{\overline{\bm{c}}}
\newcommand{\widebarbd}{\overline{\bm{d}}}
\newcommand{\widebarbe}{\overline{\bm{e}}}
\newcommand{\widebarbf}{\overline{\bm{f}}}
\newcommand{\widebarbg}{\overline{\bm{g}}}
\newcommand{\widebarbh}{\overline{\bm{h}}}
\newcommand{\widebarbi}{\overline{\bm{i}}}
\newcommand{\widebarbj}{\overline{\bm{j}}}
\newcommand{\widebarbk}{\overline{\bm{k}}}
\newcommand{\widebarbl}{\overline{\bm{l}}}
\newcommand{\widebarbm}{\overline{\bm{m}}}
\newcommand{\widebarbn}{\overline{\bm{n}}}
\newcommand{\widebarbo}{\overline{\bm{o}}}
\newcommand{\widebarbp}{\overline{\bm{p}}}
\newcommand{\widebarbq}{\overline{\bm{q}}}
\newcommand{\widebarbr}{\overline{\bm{r}}}
\newcommand{\widebarbs}{\overline{\bm{s}}}
\newcommand{\widebarbt}{\overline{\bm{t}}}
\newcommand{\widebarbu}{\overline{\bm{u}}}
\newcommand{\widebarbv}{\overline{\bm{v}}}
\newcommand{\widebarbw}{\overline{\bm{w}}}
\newcommand{\widebarbx}{\overline{\bm{x}}}
\newcommand{\widebarby}{\overline{\bm{y}}}
\newcommand{\widebarbz}{\overline{\bm{z}}}


\newcommand{\widetildebA}{\widetilde{\bm{A}}}
\newcommand{\widetildebB}{\widetilde{\bm{B}}}
\newcommand{\widetildebC}{\widetilde{\bm{C}}}
\newcommand{\widetildebD}{\widetilde{\bm{D}}}
\newcommand{\widetildebE}{\widetilde{\bm{E}}}
\newcommand{\widetildebF}{\widetilde{\bm{F}}}
\newcommand{\widetildebG}{\widetilde{\bm{G}}}
\newcommand{\widetildebH}{\widetilde{\bm{H}}}
\newcommand{\widetildebI}{\widetilde{\bm{I}}}
\newcommand{\widetildebJ}{\widetilde{\bm{J}}}
\newcommand{\widetildebK}{\widetilde{\bm{K}}}
\newcommand{\widetildebL}{\widetilde{\bm{L}}}
\newcommand{\widetildebM}{\widetilde{\bm{M}}}
\newcommand{\widetildebN}{\widetilde{\bm{N}}}
\newcommand{\widetildebO}{\widetilde{\bm{O}}}
\newcommand{\widetildebP}{\widetilde{\bm{P}}}
\newcommand{\widetildebQ}{\widetilde{\bm{Q}}}
\newcommand{\widetildebR}{\widetilde{\bm{R}}}
\newcommand{\widetildebS}{\widetilde{\bm{S}}}
\newcommand{\widetildebT}{\widetilde{\bm{T}}}
\newcommand{\widetildebU}{\widetilde{\bm{U}}}
\newcommand{\widetildebV}{\widetilde{\bm{V}}}
\newcommand{\widetildebW}{\widetilde{\bm{W}}}
\newcommand{\widetildebX}{\widetilde{\bm{X}}}
\newcommand{\widetildebY}{\widetilde{\bm{Y}}}
\newcommand{\widetildebZ}{\widetilde{\bm{Z}}}
\newcommand{\widetildeba}{\widetilde{\bm{a}}}
\newcommand{\widetildebb}{\widetilde{\bm{b}}}
\newcommand{\widetildebc}{\widetilde{\bm{c}}}
\newcommand{\widetildebd}{\widetilde{\bm{d}}}
\newcommand{\widetildebe}{\widetilde{\bm{e}}}
\newcommand{\widetildebf}{\widetilde{\bm{f}}}
\newcommand{\widetildebg}{\widetilde{\bm{g}}}
\newcommand{\widetildebh}{\widetilde{\bm{h}}}
\newcommand{\widetildebi}{\widetilde{\bm{i}}}
\newcommand{\widetildebj}{\widetilde{\bm{j}}}
\newcommand{\widetildebk}{\widetilde{\bm{k}}}
\newcommand{\widetildebl}{\widetilde{\bm{l}}}
\newcommand{\widetildebm}{\widetilde{\bm{m}}}
\newcommand{\widetildebn}{\widetilde{\bm{n}}}
\newcommand{\widetildebo}{\widetilde{\bm{o}}}
\newcommand{\widetildebp}{\widetilde{\bm{p}}}
\newcommand{\widetildebq}{\widetilde{\bm{q}}}
\newcommand{\widetildebr}{\widetilde{\bm{r}}}
\newcommand{\widetildebs}{\widetilde{\bm{s}}}
\newcommand{\widetildebt}{\widetilde{\bm{t}}}
\newcommand{\widetildebu}{\widetilde{\bm{u}}}
\newcommand{\widetildebv}{\widetilde{\bm{v}}}
\newcommand{\widetildebw}{\widetilde{\bm{w}}}
\newcommand{\widetildebx}{\widetilde{\bm{x}}}
\newcommand{\widetildeby}{\widetilde{\bm{y}}}
\newcommand{\widetildebz}{\widetilde{\bm{z}}}




\newcommand{\off}{\text{off}}

\newcommand{\ba}{\bm{a}}
\newcommand{\bA}{\bm{A}}
\newcommand{\bb}{\bm{b}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bc}{\bm{c}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bd}{\bm{d}}
\newcommand{\bD}{\bm{D}}
\newcommand{\be}{\bm{e}}
\newcommand{\bE}{\bm{E}}
\newcommand{\bff}{\bm{f}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bg}{\bm{g}}
\newcommand{\bG}{\bm{G}}
\newcommand{\bh}{\bm{h}}
\newcommand{\bH}{\bm{H}}
\newcommand{\bi}{\bm{i}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bj}{\bm{j}}
\newcommand{\bJ}{\bm{J}}
\newcommand{\bk}{\bm{k}}
\newcommand{\bK}{\bm{K}}
\newcommand{\bl}{\bm{l}}
\newcommand{\bL}{\bm{L}}
\newcommand{\bmm}{\bm{m}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bn}{\bm{n}}
\newcommand{\bN}{\bm{N}}
\newcommand{\bo}{\bm{o}}
\newcommand{\bO}{\bm{O}}
\newcommand{\bp}{\bm{p}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bq}{\bm{q}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\br}{\bm{r}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bt}{\bm{t}}
\newcommand{\bT}{\bm{T}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bU}{\bm{U}}
\newcommand{\bv}{\bm{v}}
\newcommand{\bV}{\bm{V}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bx}{\bm{x}}
\newcommand{\bX}{\bm{X}}
\newcommand{\by}{\bm{y}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\bz}{\bm{z}}
\newcommand{\bZ}{\bm{Z}}



\newcommand{\abovebX}[1]{\overset{\mathit{(#1)}}{\bX}}


\newcommand{\eG}{\bm{\mathscr{G}}}
\newcommand{\eA}{\bm{\mathscr{A}}}
\newcommand{\eB}{\bm{\mathscr{B}}}
\newcommand{\eY}{\bm{\mathscr{Y}}}
\newcommand{\eX}{\bm{\mathscr{X}}}
\newcommand{\eL}{\bm{\mathscr{L}}}
\newcommand{\weX}{\widehat{\bm{\mathscr{X}}}}
\newcommand{\weG}{\widehat{\bm{\mathscr{G}}}}

\newcommand{\widehatbA}{\widehat{\bm{A}}}

\newcommand{\mathcalV}{\mathcal{V}}
\newcommand{\dist}{\mathrm{dist}}

\newcommand{\bzero}{\mathbf{0}}
\newcommand{\kernel}{\mathbf{ker}}
\newcommand{\mathE}{\mathbb{E}}


\newcommand{\mat}[1]{\mathbf{#1}}
\renewcommand\vec{\mathbf}
\newcommand\inv[1]{#1\raisebox{1.15ex}{$\scriptscriptstyle-\!1$}}
\newcommand{\trans}[1]{\ensuremath{#1^{ \top}}}

% biconjugate decomposition
\newcommand{\brx}{\bm{R}_\gamma^{(x)}}
\newcommand{\bry}{\bm{R}_\gamma^{(y)}} 
\newcommand{\brxt}{\bm{R}_\gamma^{(x)\top}}
\newcommand{\bryt}{\bm{R}_\gamma^{(y)\top}} 
\newcommand{\bxgamma}{\bX_\gamma}
\newcommand{\bygamma}{\bY_\gamma}
\newcommand{\bugamma}{\bU_\gamma}
\newcommand{\bvgamma}{\bV_\gamma}
\newcommand{\bomegagamma}{\bOmega_\gamma}
\newcommand{\svd}{\mathrm{svd}}
